Nonconvex Regularized Gradient Projection Sparse Reconstruction for Massive MIMO Channel Estimation

Novel sparse reconstruction algorithms are proposed for beamspace channel estimation in massive multiple-input multiple-output systems. The proposed algorithms minimize a least-squares objective having a nonconvex regularizer. This regularizer removes the penalties on a few large-magnitude elements from the conventional l1-norm regularizer, and thus it only forces penalties on the remaining elements that are expected to be zeros. Accurate and fast reconstructions can be achieved by performing gradient projection updates within the framework of difference of convex functions (DC) programming. A double-loop algorithm and a single-loop algorithm are proposed via different DC decompositions, and these two algorithms have distinct computation complexities and convergence rates. Then, an extension algorithm is further proposed by designing the step sizes of the single-loop algorithm. The extension algorithm has a faster convergence rate and can achieve approximately the same level of accuracy as the proposed double-loop algorithm. Numerical results show significant advantages of the proposed algorithms over existing reconstruction algorithms in terms of reconstruction accuracies and runtimes. Compared to the benchmark channel estimation techniques, the proposed algorithms also achieve smaller mean squared error and higher achievable spectral efficiency.

==> lmmse_ls.tex <==
We adopt the minimum NMSE for LS and LMMSE estimation as baselines.
	Under the assumption of adopting optimal orthonormal pilot matrix, the minimum NMSE for LS estimation is given by \cc{cite Training-Based MIMO Channel Estimation: A Study
of Estimator Tradeoffs and Optimal Training Signals}
	\begin{equation} \label{min_nmse_ls}
		\text{NMSE}_\text{{min, LS}} = \frac{\sigma^2 N_t^2 N_r}{\mathcal{P}}
	\end{equation}
	where $\mathcal{P}=\norm{\mathbf P}_F^2$; $\sigma^2$ is the noise power at the receiver.
	
	The minimum NMSE for LMMSE estimation is given by \cc{cite Tse pp.342 eq.(5.197)}
	\begin{equation} \label{min_nmse_lmmse}
		\text{NMSE}_\text{{min, LMMSE}} = \frac{1}{1+\text{SNR}/N_t}
	\end{equation}		
	where the SNR is the signal to noise ratio per symbol.
%	, which can be calculated by $\text{SNR} = \frac{\mathcal{P}}{\sigma^2 N_t N_r}$.	
	
	To evaluate the accuracy of the proposed algorithm, we run a simulation for $1,000$ channel vector samples using the proposed SlDC-GPSR algorithm, and plot the NMSE versus SNR in Fig.\ref{res_nmse_04051650}.
	In the simulation setup, the number of BS antennas is set as $N_t=256$, and the number of user antenna is set as $N_r=1$. Therefore, channel vectors has the dimension of $256$. The pilot training length is set as $L=128$. The number of nonzero elements for a beamspace channel vector is set as $32$.
	From Fig.\ref{res_nmse_04051650} we can see the proposed algorithm can achieve lower NMSE than the LMMSE and the LS.
	
\begin{figure}[htp]    
\centering
\includegraphics[width=5.0in]{./Figures/nmse_snr_202104061059}
\caption{Normalized mean square error (NMSE) of channel reconstruction versus signal to noise ratio (SNR)}
\label{testnmse_snr_202104061059}
\end{figure}

\begin{figure}[htp]    
\centering
\includegraphics[width=5.0in]{./Figures/ratevslen04061015}
\caption{Achievable spectral efficiency R/B (b/s/Hz) versus pilot length L (symbols)}
\label{ratevslen04061015}
\end{figure}

	
	\textit{Achievable spectral efficiency:}
	In general, a trade-off exists between the channel estimation accuracy and pilot training overhead.
	To evaluate the both influences of pilot overhead and SNR penalty caused by imperfect channel estimation, the achievable spectral efficiency can be used, which is expressed as \cc{cite Tse pp.274 eq.4.218, pp.341 section 5.6}
	\begin{equation}
		\frac{R}{B} = (1-\alpha)C(\text{SNR}_\text{eff})
	\end{equation}
	where $R$ is the achievable rate; $B$ is the bandwidth; $\alpha$ is the ratio of pilot training in a coherence block duration, and it can be calculated as $L/L_c$, where $L_c$ is the length of channel coherence block; $C(\text{SNR}_\text{eff})$ is the channel capacity at the efficient SNR, 
%	and for a single user it can be calculated as $C(\text{SNR}_\text{eff}) \approx \log_2 (1+ \text{SNR}_\text{eff})$, 
	and where $\text{SNR}_\text{eff}$ is given by \cc{cite Tse pp.341 section 5.6}
	\begin{equation} \label{eff_snr}
		\text{SNR}_\text{eff} = \frac{ \text{SNR}(1-\text{NMSE})}{1+ \text{SNR} \cdot \text{NMSE}}
	\end{equation}
	
	We plot the achievable spectral efficiency $R/B$ versus the pilot length $L$ for $\text{SNR}=40\text{dB}$.
	Under the assumption of using optimal pilot matrix, we fix the training length for LMMSE and LS as $256$, which equals to the number of transmit antennas. The minimum NMSE for LMMSE and LS in \eqref{min_nmse_lmmse} and \eqref{min_nmse_ls} are adopted for calculating the efficient SNR in \eqref{eff_snr}.

